Sparse identification of nonlinear dynamics for model predictive control in the low-data limit

The data-driven discovery of dynamics via machine learning is currently pushing the frontiers of modeling and control efforts, and it provides a tremendous opportunity to extend the reach of model predictive control. However, many leading methods in machine learning, such as neural networks, require large volumes of training data, may not be interpretable, do not easily include known constraints and symmetries, and often do not generalize beyond the attractor where models are trained. These factors limit the use of these techniques for the online identification of a model in the low-data limit, for example following an abrupt change to the system dynamics. In this work, we extend the recent sparse identification of nonlinear dynamics (SINDY) modeling procedure to include the effects of actuation and demonstrate the ability of these models to enhance the performance of model predictive control (MPC), based on limited, noisy data. SINDY models are parsimonious, identifying the fewest terms in the model needed to explain the data, making them interpretable, generalizable, and reducing the burden of training data. We show that the resulting SINDY-MPC framework has higher performance, requires significantly less data, and is more computationally efficient and robust to noise than neural network models, making it viable for online training and execution in response to rapid changes to the system. SINDY-MPC also shows improved performance over linear data-driven models, although linear models may provide a stopgap until enough data is available for SINDY. SINDY-MPC is demonstrated on a variety of dynamical systems with different challenges, including the chaotic Lorenz system, a simple model for flight control of an F8 aircraft, and an HIV model incorporating drug treatment.

==> Header2.tex <==
\usepackage[top=.75in, bottom=.75in, left=.65in, right=.65in,paperwidth=8.5in,paperheight=11in]{geometry}
\usepackage[authoryear]{natbib}

\usepackage[innercaption]{sidecap}
\setlength{\parskip}{0pt} % 1ex plus 0.5ex minus 0.2ex}

%\usepackage[top=1in, bottom=1in, left=.85in, right=.85in]{geometry}
\setlength\parindent{0.25in}
\setlength{\columnsep}{.15in}
\pdfminorversion=4




==> Sec6.tex <==
\section{Conclusions}\label{Sec:Conclusion}



==> Sec7.tex <==
\section{Effect of actuation input on the training}
\begin{figure*}[tb]
	\centering
	\hfill\begin{overpic}[width=0.22\textwidth, trim = {5 35 18 0}, clip=true]{EX_LOTKA_SI_SINDYc_sine2_Actuation_OneFig}
		\put(30,60){(a) Sinusoidal}
	\end{overpic}	
	\begin{overpic}[width=0.23\textwidth, trim = {18 35 18 0}, clip=true]{EX_LOTKA_SI_SINDYc_sphs_Actuation_OneFig}
		\put(0,60){(b) Schroeder-type signal}
	\end{overpic}	
	\begin{overpic}[width=0.23\textwidth, trim = {18 35 18 0}, clip=true]{EX_LOTKA_SI_SINDYc_prbs_Actuation_OneFig}
		\put(35,60){(c) PRBS}
	\end{overpic}	
	%	\begin{overpic}[width=0.18\textwidth, trim = {18 35 18 0}, clip=true]{EX_LOTKA_SI_SINDYc_chirp_Actuation_OneFig}
	%		\put(35,60){(d) Chirp}
	%	\end{overpic}	
	\begin{overpic}[width=0.23\textwidth, trim = {18 35 18 0}, clip=true]{EX_LOTKA_SI_SINDYc_mixed_Actuation_OneFig}
		\put(35,60){(e) Mixed}
	\end{overpic}\\
	\hfill\begin{overpic}[width=0.225\textwidth, trim = {5 35 18 0}, clip=true]{EX_LOTKA_SI_DMDc_sine2_Validation_OneFig}
		\put(-15,10){\rotatebox{90}{DMDc}}
	\end{overpic}	
	\includegraphics[width=0.23\textwidth, trim = {18 35 18 0}, clip=true]{EX_LOTKA_SI_DMDc_sphs_Validation_OneFig}
	\includegraphics[width=0.23\textwidth, trim = {18 35 18 0}, clip=true]{EX_LOTKA_SI_DMDc_prbs_Validation_OneFig}
	%	\includegraphics[width=0.18\textwidth, trim = {18 35 18 0}, clip=true]{EX_LOTKA_SI_DMDc_chirp_Validation_OneFig}
	\includegraphics[width=0.23\textwidth, trim = {18 35 18 0}, clip=true]{EX_LOTKA_SI_DMDc_mixed_Validation_OneFig}\\
	\hfill\begin{overpic}[width=0.225\textwidth, trim = {5 35 18 0}, clip=true]{EX_LOTKA_SI_SINDYc_sine2_Validation_OneFig}
		\put(-15,10){\rotatebox{90}{SINDYc}}
	\end{overpic}		
	\includegraphics[width=0.23\textwidth, trim = {18 35 18 0}, clip=true]{EX_LOTKA_SI_SINDYc_sphs_Validation_OneFig}
	\includegraphics[width=0.23\textwidth, trim = {18 35 18 0}, clip=true]{EX_LOTKA_SI_SINDYc_prbs_Validation_OneFig}
	%	\includegraphics[width=0.18\textwidth, trim = {18 35 18 0}, clip=true]{EX_LOTKA_SI_SINDYc_chirp_Validation_OneFig}
	\includegraphics[width=0.23\textwidth, trim = {18 35 18 0}, clip=true]{EX_LOTKA_SI_SINDYc_mixed_Validation_OneFig}\\
	\hfill\begin{overpic}[width=0.225\textwidth, trim = {5 0 18 0}, clip=true]{EX_LOTKA_SI_NARX_sine2_Validation_OneFig}
		\put(-15,20){\rotatebox{90}{NARX}}
	\end{overpic}		
	\includegraphics[width=0.23\textwidth, trim = {18 0 18 0}, clip=true]{EX_LOTKA_SI_NARX_sphs_Validation_OneFig}
	\includegraphics[width=0.23\textwidth, trim = {18 0 18 0}, clip=true]{EX_LOTKA_SI_NARX_prbs_Validation_OneFig}
	%	\includegraphics[width=0.18\textwidth, trim = {18 0 18 0}, clip=true]{EX_LOTKA_SI_NARX_chirp_Validation_OneFig}
	\includegraphics[width=0.23\textwidth, trim = {18 0 18 0}, clip=true]{EX_LOTKA_SI_NARX_mixed_Validation_OneFig}
	\caption{Prediction performance of SINDYc models identified from different training data.
		In contrast to (a)--(d), the excitation signal in the prediction period changes in (e); thus the model's capability to generalize beyond the training data is explored.}
\end{figure*}
%\begin{figure*}[tb]
%	\centering
%	\hfill\begin{overpic}[width=0.187\textwidth, trim = {5 35 18 0}, clip=true]{EX_LOTKA_SI_SINDYc_sine2_Actuation_OneFig}
%		\put(30,60){(a) Sinusoidal}
%	\end{overpic}	
%	\begin{overpic}[width=0.18\textwidth, trim = {18 35 18 0}, clip=true]{EX_LOTKA_SI_SINDYc_sphs_Actuation_OneFig}
%		\put(0,60){(b) Schroeder-type signal}
%	\end{overpic}	
%	\begin{overpic}[width=0.18\textwidth, trim = {18 35 18 0}, clip=true]{EX_LOTKA_SI_SINDYc_prbs_Actuation_OneFig}
%		\put(35,60){(c) PRBS}
%	\end{overpic}	
%%	\begin{overpic}[width=0.18\textwidth, trim = {18 35 18 0}, clip=true]{EX_LOTKA_SI_SINDYc_chirp_Actuation_OneFig}
%%		\put(35,60){(d) Chirp}
%%	\end{overpic}	
%	\begin{overpic}[width=0.18\textwidth, trim = {18 35 18 0}, clip=true]{EX_LOTKA_SI_SINDYc_mixed_Actuation_OneFig}
%		\put(35,60){(e) Mixed}
%	\end{overpic}\\
%	\hfill\begin{overpic}[width=0.187\textwidth, trim = {5 35 18 0}, clip=true]{EX_LOTKA_SI_DMDc_sine2_Validation_OneFig}
%		\put(-15,10){\rotatebox{90}{DMDc}}
%	\end{overpic}	
%	\includegraphics[width=0.18\textwidth, trim = {18 35 18 0}, clip=true]{EX_LOTKA_SI_DMDc_sphs_Validation_OneFig}
%	\includegraphics[width=0.18\textwidth, trim = {18 35 18 0}, clip=true]{EX_LOTKA_SI_DMDc_prbs_Validation_OneFig}
%%	\includegraphics[width=0.18\textwidth, trim = {18 35 18 0}, clip=true]{EX_LOTKA_SI_DMDc_chirp_Validation_OneFig}
%	\includegraphics[width=0.18\textwidth, trim = {18 35 18 0}, clip=true]{EX_LOTKA_SI_DMDc_mixed_Validation_OneFig}\\
%	\hfill\begin{overpic}[width=0.187\textwidth, trim = {5 35 18 0}, clip=true]{EX_LOTKA_SI_SINDYc_sine2_Validation_OneFig}
%		\put(-15,10){\rotatebox{90}{SINDYc}}
%	\end{overpic}		
%	\includegraphics[width=0.18\textwidth, trim = {18 35 18 0}, clip=true]{EX_LOTKA_SI_SINDYc_sphs_Validation_OneFig}
%	\includegraphics[width=0.18\textwidth, trim = {18 35 18 0}, clip=true]{EX_LOTKA_SI_SINDYc_prbs_Validation_OneFig}
%%	\includegraphics[width=0.18\textwidth, trim = {18 35 18 0}, clip=true]{EX_LOTKA_SI_SINDYc_chirp_Validation_OneFig}
%	\includegraphics[width=0.18\textwidth, trim = {18 35 18 0}, clip=true]{EX_LOTKA_SI_SINDYc_mixed_Validation_OneFig}\\
%	\hfill\begin{overpic}[width=0.187\textwidth, trim = {5 0 18 0}, clip=true]{EX_LOTKA_SI_NARX_sine2_Validation_OneFig}
%		\put(-15,20){\rotatebox{90}{NARX}}
%	\end{overpic}		
%	\includegraphics[width=0.18\textwidth, trim = {18 0 18 0}, clip=true]{EX_LOTKA_SI_NARX_sphs_Validation_OneFig}
%	\includegraphics[width=0.18\textwidth, trim = {18 0 18 0}, clip=true]{EX_LOTKA_SI_NARX_prbs_Validation_OneFig}
%%	\includegraphics[width=0.18\textwidth, trim = {18 0 18 0}, clip=true]{EX_LOTKA_SI_NARX_chirp_Validation_OneFig}
%	\includegraphics[width=0.18\textwidth, trim = {18 0 18 0}, clip=true]{EX_LOTKA_SI_NARX_mixed_Validation_OneFig}
%	\caption{Prediction performance of SINDYc models identified from different training data.
%		In contrast to (a)--(d), the excitation signal in the prediction period changes in (e); thus the model's capability to generalize beyond the training data is explored.}
%\end{figure*}

\section{Effect of noise on the prediction performance}
\begin{figure*}[tb]
	\centering
	\hfill\begin{overpic}[width=0.345\textwidth, trim = {0 41 15 0}, clip=true]{EX_LOTKA_SI_DMDc_sphs_Validation_N3000_Eta005_STATS}
		\put(-15,15){\rotatebox{90}{$\eta=0.05$}}
		\put(50,53){DMDc}
	\end{overpic}	
	\begin{overpic}[width=0.29\textwidth, trim = {45 41 15 0}, clip=true]{EX_LOTKA_SI_SINDYc_sphs_Validation_N3000_Eta005_STATS}
		\put(38,62){SINDYc}
	\end{overpic}	
	\begin{overpic}[width=0.29\textwidth, trim = {45 41 15 0}, clip=true]{EX_LOTKA_SI_NARX_sphs_Validation_N3000_Eta005_STATS}
		\put(40,62){NARX}
	\end{overpic}\\
	\hfill\begin{overpic}[width=0.345\textwidth, trim = {0 0 15 2}, clip=true]{EX_LOTKA_SI_DMDc_sphs_Validation_N3000_Eta030_STATS}
		\put(-13,30){\rotatebox{90}{$\eta=0.3$}}
	\end{overpic}	
	\includegraphics[width=0.29\textwidth, trim = {45 0 15 2}, clip=true]{EX_LOTKA_SI_SINDYc_sphs_Validation_N3000_Eta030_STATS}
	\includegraphics[width=0.29\textwidth, trim = {45 0 15 2}, clip=true]{EX_LOTKA_SI_NARX_sphs_Validation_N3000_Eta030_STATS}
	\caption{Exemplary prediction performance when trained on noisy measurements, where $\eta$ is either $5\%$ or $30\%$.}%, for 50 noise realizations.}	
\end{figure*}

\begin{figure}[tb]
	\centering
	\psfrag{Eta}{$\eta$}
	(a)\includegraphics[width=0.3\textwidth]{EX_LOTKA_PREDPERF_sphs_N3000_noise_trainbr_noleg} %{EX_LOTKA_PREDPERF_sine2_N3000_noise}
	\hspace{0.5cm}
	(b)\includegraphics[width=0.3\textwidth]{EX_LOTKA_PREDPERF_sine2_N3000_noise_trainbr} %{EX_LOTKA_PREDPERF_sphs_N3000_noise}
	\caption{Prediction performance of the models in dependency of measurement noise
		using
		(a) a sinusoidal input or (b) a Schroeder-type excitation signal.  
		Statistics are shown for 50 noise realizations each. 
		Above the shaded region, the models do not have any predictive power.
	}
\end{figure}

\begin{figure}[tb]
	\centering
	\psfrag{DMDc}{\hspace{-.00cm}\small DMDc}
	\psfrag{SINDYc}{\hspace{-.00cm}\small SINDYc}
	\psfrag{NARX}{\hspace{-.00cm}\small NARX}
	\psfrag{Training Time [s]}{\raisebox{0.35cm}{\hspace{-0.2cm}Training time [s]}}
	\psfrag{Eta}{$\eta$}
	\psfrag{0.01}{\small 0.01}
	\psfrag{0.1}{\small 0.1}
	\psfrag{0.2}{\small 0.2}
	\psfrag{0.3}{\small 0.3}
	\psfrag{0.4}{\small 0.4}
	\psfrag{0.5}{\small 0.5}	
	\psfrag{10}{\small 10}
	\psfrag{1}{\tiny 1}
	\psfrag{0}{\tiny 0}
	\psfrag{-1}{\tiny -1}
	\psfrag{-2}{\tiny -2}
	\psfrag{-3}{\tiny -3}
	\includegraphics[width=0.45\textwidth, trim = {0 70 0 0}, clip=true]{EX_LOTKA_CTRLPERF_sphs_TrainingLength_Legend}\\
	\begin{overpic}[width=0.45\textwidth, trim = {0 0 0 0}, clip=true]{EX_LOTKA_PREDPERF_sphs_N3000_noiseM_trainbr_TrainTime_noleg}
		%		\put(-2,2){(a)}
		%	\put(55,35){\psfrag{Training Time [s]}{}\psfrag{Eta}{}\includegraphics[height=2.2cm, trim = {10 10 10 0}, clip=true]{EX_LOTKA_PREDPERF_sphs_N3000_noiseM_trainbr_TrainTimeZOOM_noleg}}
	\end{overpic}
	\caption{Training time of the models in dependency of measurement noise
		using a Schroeder-type excitation signal. Data and legend corresponding to Fig.~\ref{Fig:LOTKA:NOISE:traintimeVSnoise}.
	}
\end{figure}


%\begin{figure}[tb]
%	\centering
%\begin{overpic}[width=0.35\textwidth, trim = {0 80 0 0}, clip=true]{EX_LOTKA_CTRLPERF_sphs_TrainingLength_State_DMDc}
%%	\put(-7,2){(b)}
%\end{overpic}\\
%	\includegraphics[width=0.35\textwidth, trim = {0 80 0 0}, clip=true]{EX_LOTKA_CTRLPERF_sphs_TrainingLength_State_SINDYc}\\
%	\includegraphics[width=0.35\textwidth, trim = {0 0 0 0}, clip=true]{EX_LOTKA_CTRLPERF_sphs_TrainingLength_State_NARX}
%\caption{Controlled state trajectory in dependency of the length of the training data employed to train the model.}
%\end{figure}
%
%\begin{figure}[tb]
%	\centering
%	\begin{overpic}[width=0.25\textwidth, trim = {0 75 0 0}, clip=true]{EX_LOTKA_CTRLPERF_sphs_TrainingLength_Cost_DMDc}
%		%	\put(-7,2){(b)}
%	\end{overpic}\\
%	\includegraphics[width=0.25\textwidth, trim = {0 75 0 0}, clip=true]{EX_LOTKA_CTRLPERF_sphs_TrainingLength_Cost_SINDYc}\\
%	\includegraphics[width=0.25\textwidth, trim = {0 0 0 0}, clip=true]{EX_LOTKA_CTRLPERF_sphs_TrainingLength_Cost_NARX}
%	\caption{Cumulative cost over time in dependency of the length of the training data employed to train the model.}
%\end{figure}


\begin{figure}[tb]
	\centering
	\begin{overpic}[width=0.24\textwidth, trim = {0 80 0 0}, clip=true]{EX_LOTKA_CTRLPERF_sphs_TrainingLength_State_DMDc}
		%	\put(-7,2){(b)}
	\end{overpic}
	\begin{overpic}[width=0.24\textwidth, trim = {0 75 0 0}, clip=true]{EX_LOTKA_CTRLPERF_sphs_TrainingLength_Cost_DMDc}
		%	\put(-7,2){(b)}
	\end{overpic}\\
	\includegraphics[width=0.24\textwidth, trim = {0 80 0 0}, clip=true]{EX_LOTKA_CTRLPERF_sphs_TrainingLength_State_SINDYc}
	\includegraphics[width=0.24\textwidth, trim = {0 75 0 0}, clip=true]{EX_LOTKA_CTRLPERF_sphs_TrainingLength_Cost_SINDYc}\\
	\includegraphics[width=0.24\textwidth, trim = {0 0 0 0}, clip=true]{EX_LOTKA_CTRLPERF_sphs_TrainingLength_State_NARX}
	\includegraphics[width=0.24\textwidth, trim = {0 0 0 0}, clip=true]{EX_LOTKA_CTRLPERF_sphs_TrainingLength_Cost_NARX}
	\caption{Dependency on length of training data:
		(a) phase plot of controlled state trajectory, and
		(b) cumulative cost over time.}
\end{figure}




%\begin{figure}[tb]
%	\centering
%	\begin{overpic}[height=3cm]{./../FIGURES/EX_LOTKA_SI_SINDYc_sine2_Validation_OneFig}
%		\put(18,65){(a) Training/Validation}
%	\end{overpic}	
%	\begin{overpic}[height=3cm, trim = 1.5cm 0 0 0, clip=true]{./../FIGURES/EX_LOTKA_DynamicsControlled_cnstrnd_N5}
%		\put(28,78){(b) $N=5$} %18
%	\end{overpic}	
%	\begin{overpic}[height=3cm, trim = 1.5cm 0 0 0, clip=true]{./../FIGURES/EX_LOTKA_DynamicsControlled_cnstrnd_N10}
%		\put(28,78){(c) $N=10$}
%	\end{overpic}
%	\begin{overpic}[height=3cm, trim = 0 0 0 0, clip=true]{./../FIGURES/EX_LOTKA_MPC-SINDYc_CostComparison_All}
%		\put(18,60){(d) Cumulative cost}
%	\end{overpic}
%	\caption{Controlled Lotka-Volterra model using SINDYc for varying prediction/control horizon lengths.}
%\end{figure}



%\begin{figure*}[tb]
%	\centering
%	\includegraphics[width=0.9\textwidth, trim = 0 0 0 0.cm, clip=true]{../SCHEMATICS/ModelComparison}
%	\caption{Model identification of Lotka-Volterra model using DMDc, SINDYc and NARX.}
%\end{figure*}

%\begin{figure}[tb]
%	\centering
%	\includegraphics[height=2.9cm, trim = 0 0 0 0.cm, clip=true]{EX_LOTKA_MPC_DMDc}
%	\includegraphics[height=2.9cm, trim = 43 0 0 0.cm, clip=true]{EX_LOTKA_MPC_SINDYc}
%	\includegraphics[height=2.9cm, trim = 43 0 0 0.cm, clip=true]{EX_LOTKA_MPC_NARX}
%	\caption{Comparison of prediction and control performance for the three different models.
%		Execution times: 2.7 mins (DMDc), 1.3 mins (SINDYc),  42 mins (NARX).}
%	\label{Fig:LV:MPC_Comparison}
%\end{figure}



%\begin{figure}[tb]
%\centering
%\begin{overpic}[width=0.5\textwidth, trim = 0 0 0 0.cm, clip=true]{EX_LOTKA_SI_Comparison_Validation_sphs_sine2_Cost}
%	\put(35,29){T=1.3 min}
%	\put(35,38){T=42 min}
%	\put(35,48){T=2.7 min}
%\end{overpic}	
%\caption{Cumulative cost for MPC shown in Fig.~\ref{Fig:LV:MPC_Comparison}.}
%\end{figure}

